A Semi-Paired Approach For Label-to-Image Translation

Data efficiency, or the ability to generalize from a few labeled data, remains a major challenge in deep learning. Semi-supervised learning has thrived in traditional recognition tasks alleviating the need for large amounts of labeled data, yet it remains understudied in image-to-image translation (I2I) tasks. In this work, we introduce the first semi-supervised (semi-paired) framework for label-to-image translation, a challenging subtask of I2I which generates photorealistic images from semantic label maps. In the semi-paired setting, the model has access to a small set of paired data and a larger set of unpaired images and labels. Instead of using geometrical transformations as a pretext task like previous works, we leverage an input reconstruction task by exploiting the conditional discriminator on the paired data as a reverse generator. We propose a training algorithm for this shared network, and we present a rare classes sampling algorithm to focus on under-represented classes. Experiments on 3 standard benchmarks show that the proposed model outperforms state-of-the-art unsupervised and semi-supervised approaches, as well as some fully supervised approaches while using a much smaller number of paired samples.

==> Tables/compressed_tables.tex <==
\begin{table*}[h!]
%	\vspace{-1.5em}

	 %
	%\vspace{-0.5em}

	\setlength{\tabcolsep}{0.2em}
	\renewcommand{\arraystretch}{0.95}
	\centering
	
	\subfloat[caption 1]{\scalebox{0.90}{\begin{tabular}{l|c|cc|cc|c|cc}
    	\multirow{2}{*}{ Method } & \multirow{2}{*}{$r$} & \multicolumn{2}{c|}{ Cityscapes} &  \multicolumn{2}{c|}{ ADE20K} & \multirow{2}{*}{$r$} & \multicolumn{2}{c}{ COCO-stuff}
    	\tabularnewline
    	  &   & FID$\downarrow$  &  mIoU$\uparrow$ &   FID$\downarrow$  &  mIoU$\uparrow$ &  &  FID$\downarrow$  &  mIoU$\uparrow$ \tabularnewline
    	
    	\hline 
    	
    	\small{} USIS	& 0.0  &  0.0 &  0.0 &  0.0 &  0.0 &  0.0  & 0.0 & 0.0 \tabularnewline 
    	
    	%\arrayrulecolor{lightgray}
    	
    	 \hline
    	
    	\small{} OASIS	& \multirow{3}{*}{$20$} &  0.0 &  0.0 &  0.0 &  0.0 &   \multirow{3}{*}{$0.5$} & 0.0 &  0.0   \tabularnewline
    	
    	\small{} TCR	&  &  0.0 &  0.0 &  0.0 &  0.0 & & 0.0 &  0.0    \tabularnewline
    	
    	\small{} Ours	&  &    0.0 &  0.0 &  0.0 &  0.0 & & 0.0 &  0.0     \tabularnewline
    	
    	\hline
    	
    	\small{} OASIS	& \multirow{3}{*}{$40$} &    0.0 &  0.0 &  0.0 &  0.0 &  \multirow{3}{*}{$1$} &     0.0 &  0.0 \tabularnewline
    	
    	\small{} TCR	&  &  0.0 &  0.0 &  0.0 &  0.0 & & 0.0 &  0.0    \tabularnewline
    	
    	\small{} Ours	&  &    0.0 &  0.0 &  0.0 &  0.0 & & 0.0 &  0.0     \tabularnewline
    	
    	\hline
    	
    	\small{} OASIS	& \multirow{3}{*}{$60$} &    0.0 &  0.0 &  0.0 &  0.0 &  \multirow{3}{*}{$5$} &     0.0 &  0.0 \tabularnewline
    	
    	\small{} TCR	&  &  0.0 &  0.0 &  0.0 &  0.0 & & 0.0 &  0.0    \tabularnewline
    	
    	\small{} Ours	&  &    0.0 &  0.0 &  0.0 &  0.0 & & 0.0 &  0.0     \tabularnewline
    	
    	\hline
    	
    	\small{} OASIS	& 100  &  0.0 &  0.0 &  0.0 &  0.0 &  0.0  & 0.0 & 0.0 \tabularnewline 
    	
    	
		
		\end{tabular}}}
		\quad
		\subfloat[caption 2]{
		\vspace{1em}
		\begin{tabular}{l|cc}
		\centering
         Method & FID & mIoU  \\ 
         \hline
        OASIS                                      & 52.19 & 42.8  \\
        \hline
        OASIS + USIS                               & 50.52 & 40.27 \\
        Ours w/o $\mathcal{L}_{fm}$                & 51.37 & 39.88 \\
        Ours w/o $\mathcal{L}_{VGG}$               & 51.37 & 39.88 \\
        Ours w/o weighted sampling                 & 54.78 & 35.74 \\
        Ours w/o $\Du$                             & 54.78 & 35.74 \\
        \hline
        Ours                                       & 54.78 & 35.74 \\
        \end{tabular}}
        
	\vspace{-1em}
\end{table*}


